Just Undo It: Exploring Undo Mechanics in Multi-User Virtual Reality

With the proliferation of VR and a metaverse on the horizon, many multi-user activities are migrating to the VR world, calling for effective collaboration support. As one key feature, traditional collaborative systems provide users with undo mechanics to reverse errors and other unwanted changes. While undo has been extensively researched in this domain and is now considered industry standard, it is strikingly absent for VR systems in research and industry. This work addresses this research gap by exploring different undo techniques for basic object manipulation in different collaboration modes in VR. We conducted a study involving 32 participants organized in teams of two. Here, we studied users' performance and preferences in a tower stacking task, varying the available undo techniques and their mode of collaboration. The results suggest that users desire and use undo in VR and that the choice of the undo technique impacts users' performance and social connection.

==> content/03_concept.tex <==
\section{Concept}
\label{sec:concept}
%allgemeine Idee vorstellen
% keine "technischen Details"
% Um die lücke da zu schließen zwischen den Extrema zu überbrücken




==> content/09_acks.tex <==
\begin{acks}
	% This work has been funded by the European Research Council (ERC) under the European Union’s Horizon 2020 research and innovation programme with the ERC Consolidator Grant no. 683008.
\end{acks}

==> img/TaskPOVCOL.tex <==
\begin{figure*}[tb!]
    \vspace{2em}
	\includegraphics[width=\linewidth]{img/met/Task_POV_COL.jpg}
	\caption{Participants perspective during the \ivCollaborative{} task. The center of the image shows the stacking area, on which participants have to place the building blocks. The stairs around the stacking area can be used by participants to reach the top of the tower also for increased heights. The avatar of the other player is represented by one sphere for the head and two smaller spheres for the hands. In the back a "screen" displays the remaining time to construct the tower. Not in the picture is the area to pick up the building blocks. In this case, participants already stacked 7 blocks successfully.}

 \Description[Point of View of one participant into the collaborative game environment]{Point of View of one participant into the collaborative game environment. The center of the image shows the stacking area, on which participants have to place the building blocks. The stairs around the stacking area can be used by participants to reach the top of the tower also for increased heights. The avatar of the other player is represented by one sphere for the head and two smaller spheres for the hands. In the back a "screen" displays the remaining time to construct the tower. Not in the picture is the area to pick up the building blocks. In this case, participants already stacked 7 blocks of different color and shape successfully}
	\label{fig:Task_POV_COL}
\end{figure*}


%FIG 3

==> img/task_top_old.tex <==
\begin{figure*}[ht!]

    
    \begin{minipage}[t]{.5\linewidth}
		\includegraphics[width=0.8\linewidth]{img/met/Task_DIV.jpg}
        \centering
		\subcaption{Top view for \ivDivided{} task{}}
        \label{fig:task_top_divOLD}
	\end{minipage}%
    \begin{minipage}[t]{.5\linewidth}
		\includegraphics[width=0.8\linewidth]{img/met/Task_COL.jpg}
        \centering
		\subcaption{Top view for \ivCollaborative{} task }
        \label{fig:task_top_colOLD}
	\end{minipage}%
 
	\caption{(a) Top view of the task environment for the \ivDivided{} task. A transparent wall separates the game area to prevent interference between two players. Each player has their own stacking area as well as spawn area of the building blocks. (b) Top view of the task environment for the \ivCollaborative{} task. The players share one stacking and block spawning area.}
	
    \Description[Figure showing the task areas for the two different collaboration modes]{A two part figure showing top views of the task environment. The main components are the stacking area to place the building blocks, the block spawning area where new blocks appear and a "screen" for the timer. The left subfigure shows the top view of the task environment for the divided task. A transparent wall separates the game area to prevent interference between two players. Each player has their own stacking area as well as spawn area of the building blocks. The right subfigure shows the top view of the task environment for the collaborative task. Here the players share one stacking and block spawning area.}
	\label{fig:TaskEnvironmentOLD}
\end{figure*} 




